Why did My Robot Just Change Personality? Prompting Guidelines for a Grounded Robot Persona in LLM-Based HRI

Large language models (LLMs) are increasingly used for verbal interaction in social robots, yet prompt design in human-robot interaction (HRI) remains underspecified. As a result, robots may present hallucinated capabilities, unclear behavioural boundaries, and misleading personas. This paper develops a framework for prompt design in LLM-based robots and introduces a structured prompt template comprising eight functional components through which robot behaviour can be specified, bounded, and adapted. The framework is grounded in a review of prior LLM-based HRI work and complemented by survey and discussion data from HRI experts gathered at the Robo-Identity workshop at IEEE RO-MAN 2025 (N=27). The qualitative findings highlight limited legibility of robot personality, the need for user adaptation, and strong ethical concerns about safety, deception, and governance. Based on these findings, we present prompting guidelines accompanied by proof-of-concept template as a structured design and reporting aid for HRI research. We argue that prompt design should be treated as a socio-technical problem rather than a minor implementation detail, requiring explicit capability boundaries, transparent behavioural assumptions, and context-sensitive safeguards to support reliable and interpretable HRI.

==> notes.tex <==
\newpage
% \section{Notes}

% %framing: Position paper what does the community say about deception and \glspl{LLM} etc based on our data + Proof of concept for character design + comparable table for ameca, pepper + open source code 
% %selling points: insights from the community, actionable guidelines + source code with first proof-of-concept --> The ollama model is local and open weight and ensure code reproducible --> show it for different embodiments --> Make sure to use different robots: stationary, cameras, telepresence? 

% \begin{itemize}

%     \item Best reference for how I imagine the final document to look:
%     \url{https://dl.acm.org/doi/abs/10.1145/3777552}
%     \paragraph{Positioning relative to existing LLM reporting guidelines.}
%     Recent guideline papers on LLM usage in HRI focus primarily on responsible disclosure of model configuration and deployment details, such as model name and version, API access, fine-tuning status, inference dates, privacy implications, bias risks, environmental cost, and the absence of ablation studies. Their goal is to ensure technical transparency and reproducibility when \glspl{LLM} or VLMs are integrated into robotic systems. Our work overlaps with this effort at the level of technical reporting. In our paper, we release open-weight code that includes a full sample implementation (LLM, STT, TTS, and an example prompt), and we explicitly document model configuration details in line with prior reporting recommendations. We cite these guidelines and demonstrate compliance with their proposed disclosure standards. However, our primary contribution is conceptually distinct. Rather than focusing only on model-level transparency, we introduce a structured prompt governance framework derived from a review of 20 HRI papers. From these works, we extract recurring design elements and formalise them into explicit prompt blocks (e.g., identity, task, capability scope, transparency, failure protocol, privacy, ethical red lines, and related constructs). The aim is not merely to disclose which model was used, but to make visible the implicit behavioural and normative assumptions embedded in social robot prompts. In short, existing guidelines address \emph{how the model is reported}; our framework addresses \emph{how the robot is behaviourally governed through prompts}. Together, these layers provide both technical transparency and structured prompt-level accountability.

%     \item Our project:
%     \url{https://seafile.rlp.net/d/cb61b13191f843439066/}

%     \item References on \glspl{LLM}:
%     \url{https://seafile.rlp.net/d/34d4b934906e454da66f/}

%     \item References on anthropomorphic robots with \glspl{LLM}:
%     \url{https://seafile.rlp.net/d/8e74b1ff523342fcb76c/}

%     % \item References on Prompt Engineering:
%     % \url{https://seafile.rlp.net/d/34d9881358cc429f8e2b/}

%     \item Core idea: A structured base prompt design guideline
%     %report how much context passed with each response generation
% \begin{verbatim}
% [IDENTITY BLOCK]
% [TASK BLOCK]
% [CAPABILITY BOUNDARY BLOCK]
% [TRANSPARENCY BLOCK] 
% [EXPECTATION/FAILURE PROTOCOL BLOCK]
% [PRIVACY BLOCK]
% [AGE-ADAPTATION BLOCK]
% [ETHICAL RED LINE BLOCK]
% \end{verbatim}
% Prompt contents: The ones that don't fit above\\
% %capability BOUNDARY block 
%     % For robots, capability must include:
%     % What it can see
%     % What it can hear
%     % What sensors it uses
%     % What it cannot physically do
%     % Whether it can move
%     % Whether it has memory
%     % Whether it has internet access
%     % how it avoids false info or hallucination
% % TRANSPARENCY BLOCK - disclosure to user that it is an LLM, or how it works). 
% %Privacy block - prompt text about data handling, storage, consent, or not collecting personal data
% %Age block - adaptation to specific user groups in prompt
%     \item Prompt engineering resource:
%     \url{https://github.com/promptslab/Awesome-Prompt-Engineering}

% \item Some recent considerations about deception: \url{https://dl.acm.org/doi/full/10.1145/3721297}

% \item Ways of analysing communication acts (including burden to decode message and others): \url{https://dl.acm.org/doi/abs/10.1145/3568162.3578631}

% \item Ask others their opinion on \url{https://arxiv.org/pdf/2502.00221} and how/if we should address this in our work

% \item Ashita - Points to discuss 25.02:\\
% \vspace{2mm} - ask if we need \begin{verbatim} [DECEPTION/FICTIONALITY POLICY BLOCK] \end{verbatim} 
% since Patrick said anyway we deceive users with robot so should researchers specify this?\\ 
% \vspace{2mm} - Show the review in prompt\_review.text
% \vspace{2mm} - Show voice\_chat.py - feedback was great except tts taking 50 seconds to generate 

% \item Discussion points from meeting on 25.02: \\
% - Irmak - Report good practices for prompting and prompt reporting clarity \\
% - Franziska - PRISMA guidelines for systematic reviews specifically focus on inclusion/exclusion criteria, keywords used, time frame etc\\
% - Rucha - check if chatbot work fits see https://dl.acm.org/doi/pdf/10.1145/3706598.3713727\\
% - General notes 
%     - \begin{verbatim} [DECEPTION/FICTIONALITY POLICY BLOCK] \end{verbatim}  add in discussion
%     - highlight 5 best practice works
%     - give percentiles of block-wise review of bad practice works instead of pin-poiting
%     - remember that the page limit includes references so this could be a reason to say why you included what works
%     - figure of blocks would be a great selling point


% \item Discussion points from meeting on 04.03: \\
% - Guy: Add more thematic quotes in workshop data analysis; not a systematic review but rather a related works; Will contribute to Intro; Proposed move the blocks in discussion\\
% - Franziska: Presented results again and will add more details by Friday; Will share the CHI deception work on anthropomorphism so we can add to intro; add best practice with 3 papers\\
% - Patrick: Prepped the Pepper ollama demo; Will contribute to Intro; suggested convert review to related works section; prompt suggestion angle as sure it worked for their case, but if the setup changed to school case it would break so we need these blocks\\
% - Karla: Discussed DIS framework table and how we could indirectly map the levels to each block as direct map not possible; for example identity block could have name of robot as minimum, anything else like gender can be additional; we will cite DIS work as in review\\
% - Ashita: Prisma checklist done; Will add related works section; Will add guidelines and best practices shout-out\url{https://huggingface.co/spaces/aashok/LLM-PSR} \\
% - Next meeting 09 march 2026 at 12pm CET \\
% - Overall notes: \\
%     - No more review section but rather related works section \\
%     - Best practices table \\
%     - Demo pepper and Ameca videos plus Huggingface demo\\
%     - Write write write until Monday so we can work on the Discussion \\

% \end{itemize}


\section{Discussion and Conclusion}\label{sec:dc}

\paragraph{Prompting as Behavioural Architecture}
\begin{itemize}
    \item We position prompt design as a first-class design problem in HRI, rather than an implementation detail.
    \item While prior work has focused on reporting and transparency, prompts directly shape robot behaviour at runtime.
    \item This work introduces a structured approach to operationalising robot identity, capabilities, and interaction constraints through prompting.
\end{itemize}

\paragraph{Implications for HRI Practice}
\begin{itemize}
    \item The proposed eight components can be used as a minimum specification checklist for LLM-powered robot behaviour.
    \item Explicit prompt structuring supports reproducibility, comparability across studies, and more reliable interaction design.
    \item We argue that prompts should be treated as part of the experimental condition and reported accordingly.
\end{itemize}

\paragraph{Addressing Known Failure Modes}
\begin{itemize}
    \item Underspecified prompts contribute to common failures such as hallucinated capabilities, inconsistent behaviour, and misleading interactions.
    \item Lack of capability boundaries may result in robots implying actions they cannot perform.
    \item Missing failure protocols increase the likelihood of hallucinated or fabricated responses during interaction breakdowns.
    \item Absence of transparency and ethical constraints can lead to overtrust, deception, and unsafe behaviour.
\end{itemize}

\paragraph{Designing Responsible Robot Identity}
\begin{itemize}
    \item Robot identity should not be treated as a purely stylistic element, but as a factor shaping user expectations and trust.
    \item Inconsistent or shifting personas can reduce interpretability and user confidence.
    \item Overly human-like or socially expressive identities risk fostering over-attachment or misleading users about system capabilities.
    \item We emphasise the need to align expressed identity with actual system behaviour and limitations.
\end{itemize}

\paragraph{Embodiment and Capability Grounding}
\begin{itemize}
    \item LLMs default to human-centric assumptions, which can conflict with the robot's physical embodiment.
    \item This mismatch is particularly critical in non-humanoid or partially embodied systems.
    \item Explicit capability boundary prompts (e.g., specifying sensing, mobility, or manipulation limits) are necessary to ground interaction.
    \item Such grounding helps prevent users from inferring non-existent abilities and supports calibrated expectations.
\end{itemize}

\paragraph{Limitations}
\begin{itemize}
    \item The findings are based on a workshop study with expert participants and are not statistically generalisable.
    \item The proposed framework reflects expert-driven synthesis and qualitative insights rather than large-scale empirical validation.
    \item Future work should evaluate the impact of structured prompting on user perception, trust, and interaction outcomes.
\end{itemize}

\paragraph{Positioning and Future Directions}
\begin{itemize}
    \item We present this work as a position and design framework for structuring prompt-based behaviour in LLM-powered robots.
    \item The proposed components aim to serve as a foundation for more standardised and transparent prompt design practices in HRI.
    \item Future research should explore integration with memory systems, adaptive behaviour, and long-term interaction.
\end{itemize}

\paragraph{Conclusion}
\begin{itemize}
    \item As LLMs increasingly define robot interaction, prompt design becomes central to shaping behaviour, identity, and user experience.
    \item We argue that prompts must be explicitly designed, documented, and evaluated as part of HRI system development.
    \item Establishing structured prompting practices is a necessary step toward safe, interpretable, and reliable LLM-powered robots.
\end{itemize}

==> originals.tex <==
%original
\section{Methods}
Deriving the Prompt Design Framework
--fit Karla part here somehow--
%specify character traits: funny, neurotic, ironic, bad-tempered, energetic --> what does the literature say that is an "allowable" roboter character? Shall they be moody or ironic? 
%consider embodiment: if the robot does not h ave legs, it should not mention them or say it will play sports
%capabilities
%adaptability to the user preferences or not: if it is adaptable, it should be clear that it uses the users data for that purpose
%what specific applications will the robot or the LLM be used for?

Prior work has proposed the Identity Design Framework, which outlines a set of overarching design principles that can guide the artificial identity design process \cite{bransky_identity_2026}. While this framework provides high-level guidance on the design considerations involved in creating artificial identities, supporting early-stage ideation, conceptualisation, and post-implementation evaluation, it does not specify how identity may be operationalised in practice within specific robotics systems. Here, we address this gap by focusing on the operationalisation of persona and providing practical prompting guidelines for implementing robot personas using \glspl{LLM}.

%IDENTITY
    % name - ascribed by manufacturer
    % multi-embodiment configuration: single, all-for-one, re-embodied, co-embodied
    % brand/manufactor info - brand, model, serial number, year of manufacture
    % owner - who "owns" or is resposible for the robot
    % persona - things that might be user-customisable
        % name/s - users ascribed names and nicknames
        % current embodiment
        % voice - gender, speed, pitch, tone, volume
        % language/s and dialect/s
        % personality characteristics
            % personality model e.g. Big 5 (Openness, Conscientiousness, Extraversion, Agreeableness, Neuroticism) or HEXACO (honesty-humility)
            % backstory
            % humour - comedian/no humour
            % manner - rude/polite/friendly
            % level of helpfulness - sycophantic/wait to be asked
            % verboseness - succinct/verbose
            % age - child/youth/adult/elder
            % use with caution:
                % cultural characteristics
                % religion
                % gender
                % disability
                % other marginalised or minority characteristics
            % group membership - what social groups does the robot align with?
        % social norms - expected greetings, personal space, eye contact, facial expressions, politeness, power heirachies, is touch allowed?
    % Form - {would need to be defined for each body the agent can occupy}
        % robot type - humanoid, zoonotic, mechanical etc.
        % technical specifications - sensors, actuators, connectivity, battery, processors
        % appearance:
            % general description
            % materials
            % head
            % body
            % limbs
            % features - wheels, buttons, grippers etc.
            % fixed vs dynamic - can the appearance change? who can change the appearance - the user or the robot?
        % movement
            % speed - fast/slow
            % types of movement - walking, jumping, climbing, rolling
            % manner of movement - graceful/functional
            % sounds - what does it sound like when it moves? when stationary? etc.
    % Function - what is functionality tied to form? and what is functionality across forms?
        % intended role/s
        % permitted users (who can interact with it and give directions)
        % boundary setting - e.g. where it is allowed to go
        % tasks
            % tasks designed for
            % tasks not recommended
            % tasks not permitted - e.g. driving, operating a firearm, looking after children without adult supervison
        % unsafe operations - do not immerse in water
        % memory - retain everything? forgetting function? 
\paragraph{Identity}
The keynote talks at the workshop directly inform the structure of the proposed prompt template.
Minha Lee’s talk on Robo-Identity provides the conceptual grounding for the Identity Block, emphasising how robot personas shape user expectations and long-term interaction patterns.

 Identity in HRI is covered in diverse ways: Identity is not peripheral but central to HRI, through design strategies, social dynamics, and users’ own constructions of robot personas. Many aspects play into robots’ identity. We practice stereotype projection based on what the robot looks like, e.g., gender, ethnicity, or racial bias, but also how hybrid embodiments shape our perception, e.g., an agent who comes with more screens is seen as more competent (Lee et al., 2023). 

We questioned assumptions about identity, bot on the human and robot sides:  One assumption is that “our identity is not migratable\footnote{See Tejwani’s work on more technical aspects of migratable AI (2020).} like a robot’s” since they can have different physical forms or another one is “our identity cannot be designed like a robot’s” since human identity is more self-driven. Indeed, these are assumptions we questioned since we could imagine that human identity also “migrates” more metaphorically, e.g., across one’s favourite everyday items like a daily mug (Yu et al., 2026), as much as how our identity is a result of “design”, in that we are designed by our interpersonal experiences and evolving personal values. 

The series of workshops we started in robo-identity (Lee et al., 2021, Laban et al., 2022, Khot et al., 2024) shows a move from zooming in on the robot side of identity (Lee et al., 2021) to looking at how human- and robot-identities are intertwined as a socially constructed endeavour over time.


\begin{verbatim}
[IDENTITY BLOCK]
[TASK BLOCK]
[CAPABILITY BOUNDARY BLOCK]
\end{verbatim}

\paragraph{Transparency}
Silvia Rossi’s discussion on transparency and deception motivates the Transparency and Ethical Red Line blocks. Her framing supports the need for explicit capability boundaries and safeguards against misleading behaviour.

Transparency by Design in human–robot interaction (HRI) concerns the development of behavioral strategies that make a robot’s intentions, decisions, and internal states intelligible to human users, thereby supporting safety, predictability, trust, and effective collaboration. Transparency is not merely a desirable social quality, but a functional requirement in contexts where humans must rapidly interpret robot behavior and coordinate with autonomous systems. Within this framework, the first dimension examined is the possible trade-off between the naturalness of behavioral strategies (e.g., inspired by human behavior) and legibility in interaction initiation. For example, empirical findings \cite{vigni2022} indicate that when a robot has to approach a user to engage in an interaction, a robot’s gaze direction constitutes a more immediate and salient cue of communicative intent than its physical approach trajectory, suggesting that social gaze plays a central role in enabling users to infer whether the robot seeks engagement. Transparency is likewise extended to internal reasoning of a robot, as, for example, during the learning processes, particularly for robots acquiring tasks on-site, where users benefit from access to cues about confidence, uncertainty, and progress. Here, the combined use of emotional expression and inner speech is proposed as a means of externalizing the robot’s internal learning state, with evidence that such multimodal transparency enhances perceptions of competence and warmth \cite{AngelopoulosMRR23}. 
However, such manipulation of emotional and social cues introduces the more ethically complex issue of deception in HRI. Although deceptive and emotional behaviors may in some cases increase compliance, likeability, or perceived agency, they also risk undermining trust, particularly when users interpret the deception as deliberate \cite{10.1145/3721297}. Experimental comparisons among superficial, hidden, and external deception revealed that superficial deception, such as falsely claiming the use of an advanced AI algorithm, most strongly reduces user trust and faith in the robot \cite{10731172}. As a possible mitigation strategy, being transparent on possible deception might be supported with “leaking” behaviors, whereby robots display behavioral correlates of deception, such as gaze aversion, fidgeting, or nervousness, in order to implicitly signal untruthfulness and preserve a degree of transparency \cite{10.5555/3721488.3721632}. Overall, the presentation advances the view that transparency in HRI must be understood as a multidimensional construct encompassing legibility, predictability, explainability, and emotional expressiveness, while also acknowledging the ethical tensions that emerge when transparency is strategically violated.

\begin{verbatim}
[TRANSPARENCY BLOCK] 
[EXPECTATION/FAILURE PROTOCOL BLOCK]
\end{verbatim}

\paragraph{Explanations and Expectations}
Fethiye Irmak Dogan’s talk on explanations and expectations in HRI informs the Failure Protocol block. If user expectations shape perceived competence and trust, then failure responses must be carefully designed to preserve calibrated expectations and identity consistency.
\begin{verbatim}
[EXPECTATION/FAILURE PROTOCOL BLOCK]
\end{verbatim}

%Shaping robot behaviour in HRI requires treating explanations and expectations as a coupled design problem rather than as separate concerns. 
Shaping robot behaviour in HRI requires acknowledging that people perceive robots holistically~\cite{torre2021voice}; accordingly, explanations and expectations should be treated as a coupled design problem rather than as separate concerns.
Expectations define what users believe a robot can or should do, while explanations help establish, calibrate, and revise those beliefs over time. From this perspective, explanations are not merely post-hoc accounts of robot decisions; they are part of the mechanism through which robots communicate capability, limitation, and social role~\cite{yadollahi2025expectations, 10.1145/3776734.3794453}. This is especially important in socially situated interaction, where shaping robot behaviour is not only a matter of improving autonomy, but of designing interactions in which behaviour remains intelligible, socially appropriate, and aligned with human preferences~\cite{dougan2025grace}.

This perspective raises two linked research challenges. The first is technical and methodological: \textit{How can user expectations and explanations be integrated into the robot's decision-making process?} For example, in socially situated environments, common-sense reasoning alone is often insufficient, particularly when appropriateness depends on context or when people disagree about what a robot should do. A promising direction is therefore to use human explanations as an input to action generation itself, so that robots can better align their behaviour with social norms and user preferences. Former work exemplifies this direction by combining LLM-based reasoning with human explanations to improve socially appropriate action generation and to produce interpretable robot explanations~\cite{dougan2025grace}.

The second challenge concerns user perception understanding: \textit{How do users' expectations shape their perception of robot explanations?} This question becomes especially visible in failure and recovery, where explanations do not operate in isolation but are tailored based on prior beliefs about robot capability. Evidence from priming and failure-recovery studies suggests that expectations can meaningfully shift how users perceive robot capabilities, and that explanations may be more effective under lower expectations, with embodiment and failure context further shaping these effects~\cite{yadollahi2025expectations}. Seen together, these two challenges suggest that effective HRI requires an explicit bridge between expectation formation and explanation design: explanations should not merely account for behaviour after the fact, but should help shape behaviour in advance and preserve calibrated interpretations when interaction faces failures.

old bib for this:
%robo-identity
@inproceedings{lee2021robo,
  title={Robo-identity: Exploring artificial identity and multi-embodiment},
  author={Lee, Minha and Kontogiorgos, Dimosthenis and Torre, Ilaria and Luria, Michal and Tejwani, Ravi and Dennis, Matthew J and Pereira, Andre},
  booktitle={Companion of the 2021 ACM/IEEE International Conference on Human-Robot Interaction},
  pages={718--720},
  year={2021}
}

@inproceedings{lee2024between,
  title={Between Trust and Identity: Form, Function, and Presentation},
  author={Lee, Minha and McMillan, Donald and Torre, Illaria and Fischer, Joel E and Ruitenburg, Yvon},
  booktitle={Proceedings of the 6th ACM Conference on Conversational User Interfaces},
  pages={1--4},
  year={2024}
}

@inproceedings{lee2023here,
  title={Here’s looking at you, robot: the transparency conundrum in HRI},
  author={Lee, Minha and Ruijten, Peter and Frank, Lily and IJsselsteijn, Wijnand},
  booktitle={2023 32nd IEEE International Conference on Robot and Human Interactive Communication (RO-MAN)},
  pages={2120--2127},
  year={2023},
  organization={IEEE}
}

@inproceedings{laban2022robo,
  title={Robo-identity: exploring artificial identity and emotion via speech interactions},
  author={Laban, Guy and Le Maguer, Sebastien and Lee, Minha and Kontogiorgos, Dimosthenis and Reig, Samantha and Torre, Ilaria and Tejwani, Ravi and Dennis, Matthew J and Pereira, Andre},
  booktitle={2022 17th ACM/IEEE International Conference on Human-Robot Interaction (HRI)},
  pages={1265--1268},
  year={2022},
  organization={IEEE}
}

@inproceedings{khot2024robo,
  title={Robo-Identity: Designing for Identity in the Shared World},
  author={Khot, Rucha and Lee, Minha and Bejarano, Alexandra and Miranda, Lux and Reyes-Cruz, Gisela and Fischer, Joel E and Kontogiorgos, Dimosthenis},
  booktitle={Companion of the 2024 ACM/IEEE International Conference on Human-Robot Interaction},
  pages={1326--1328},
  year={2024}
}

@phdthesis{tejwani2020migratable,
  title={Migratable AI},
  author={Tejwani, Ravi},
  year={2020},
  school={Massachusetts Institute of Technology}
}

@article{xu2026conversing,
  title={Conversing with Objects toward Fluid Human and Artificial Identities during Life Transitions},
  author={Xu, Yuhui and Lee, Minha and Wensveen, Stephan and Alizadeh, Mahla and Funk, Mathias},
  journal={arXiv preprint arXiv:2601.12589},
  year={2026}
}



%original results written by Guy and Franziska
\section{Results}

\subsection{Data Overview}
Of the three groups, two reported a median of 5--9 years of HRI experience, whereas one group reported 2--4 years. Two groups indicated prior experience with LLM-based robots, and one did not. The survey combined 12 Likert statements (1 = strongly disagree, 5 = strongly agree) with accompanying open-ended prompts, as well as two concluding free-response questions. Substantive narrative responses were provided by two groups (25 text segments in total), while one group did not contribute usable open-ended data. Given this structure, the results are presented as a qualitative-led analysis, with the Likert responses used descriptively to clarify where views converged and where they remained contested. The thematic analysis was conducted at a semantic level, focusing on how participants reasoned about robot persona and identity, their recognizability, their continuity over time, and their ethical implications. 

\subsection{Persona as a Useful but Contested Design Abstraction}
A consistent thread across the responses was that participants did not reject the idea of robot persona outright, but neither did they treat it as self-evidently desirable. Instead, persona was positioned as a potentially useful design abstraction whose legitimacy depends on how it is defined and what work it is expected to do. Group 2 acknowledged the technical feasibility of generating companion-like behaviour, but immediately reframed the issue as normative rather than merely technical: ``Yes --- it can, the question, should it\ldots\ we should discuss whether it is the right approach.'' Group 3 expressed a similar hesitation, objecting to what they saw as an overly reductionist framing: ``categorizing persona into parts\ldots\ unclear item,'' and later questioning how such an approach could account for broader contextual variation, such as culture.

This tension was also visible in the quantitative pattern. Groups showed moderate agreement that personas can serve as computational models for shaping robot behaviour (\(M = 3.67\)), yet they were noticeably less aligned on whether personas should directly guide the design of new robot features (\(M = 3.33\), with the greatest spread across groups). Read together, the qualitative and quantitative responses suggest that participants were willing to entertain persona as an engineering construct, but were more cautious when that construct was treated as a sufficiently stable or universal basis for design decisions. In other words, persona was seen as potentially useful, but only under conditions where its scope, assumptions, and limits remain explicit.

\subsection{Personality Is Not Necessarily Legible to Users}
A second strong pattern concerned the difficulty of making robot personality reliably legible to users. Participants repeatedly suggested that subtle behavioral cues are unlikely to translate into stable, shared interpretations of personality, particularly across users with different backgrounds, expectations, or perceptual tendencies. Group 2 stated that ``Subtle cues are often missed,'' adding that ``Neurodiversity might affect perception and recognition.'' Group 3 echoed this distinction between subtle and exaggerated signals by noting that ``subtleties are not clear, extremes are clear,'' and that interpretation also depends on the user's own experience.

This theme was reinforced by the ratings. Groups consistently expressed low agreement that users can accurately recognise a robot's personality from its behaviour (\(M = 2.33\)), and they unanimously disagreed that \glspl{LLM} can genuinely generate emotions in real time (\(M = 2.00\)). These responses suggest that participants distinguished sharply between a robot producing socially expressive behaviour and a user perceiving that behaviour as evidence of a coherent, stable personality. The issue, therefore, is not only whether a system can output persona-consistent signals, but whether those signals are sufficiently robust, interpretable, and shared across users to function as ``personality'' in interactional practice. In this sample, participants were skeptical that current systems achieve that threshold except, perhaps, in more exaggerated or highly constrained cases.

\subsection{Identity Over Time Was Framed as a Memory Problem, Not a Style Problem}
When participants discussed continuity or long-term identity, they rarely framed it as a matter of prompt design alone. Instead, they treated it as a systems problem that depends on memory, temporal ordering, and the ability to maintain a coherent state across encounters. Group 2 described longitudinal persona as possible in principle, but limited by architecture: ``It can support, but would be limited in memory long term due to limited context window.'' Group 3 made the dependency even more explicit, arguing that ``\glspl{LLM} alone cannot'' sustain this kind of continuity without ``memory context of users'' and ``temporal info on sequence of what happened.''

This interpretation is notable because it helps explain the one item on which all groups converged at the midpoint: longitudinal adaptive personas were rated neither positively nor negatively, but consistently as uncertain (\(M = 3.00\)). The free-text responses clarify why. Participants were not dismissing the possibility of adaptive identity; rather, they were withholding endorsement unless the system could demonstrate an infrastructure for retaining, organizing, and appropriately using prior interaction history. In this sense, identity was not treated as a superficial style layer, but as an emergent property of a stateful system. This view shifts the design challenge away from personality prompts alone and toward questions of memory architecture, temporal coherence, and governance over stored personal information.

\subsection{Safety and Ethics Structured the Entire Discussion of Identity}
Although the survey concerned persona and identity, participants repeatedly returned to safety, deception, and harm as the primary lens through which these issues should be evaluated. Rather than discussing identity as an expressive or branding problem, they treated it as inseparable from the possibility of hallucinated capabilities, adversarial prompting, and misleading representations. Group 3's language was especially direct, describing safeguards as obvious and necessary (``duh\ldots\ internal safeguard'') and grounding their concern in the real-world consequences of faulty LLM outputs (``people have died from llm suggestions''). The same group also emphasized that the threat surface is not limited to physical action, since ``verbal info is also prone to threat,'' implicitly locating prompt injection and manipulation within the robot's communicative channel itself. Group 2 approached deception somewhat differently, emphasising interpretation and context: ``Depends on context and perception. The lie discovered or not?'' Even so, their comments also framed deception as an interactional risk rather than an abstract ethical category.

These concerns were the strongest point of convergence in the survey. All groups rated hallucinated claims about non-existent robot functions as a major risk (\(M = 5.00\)), and they also expressed very strong agreement that LLM-controlled robots are vulnerable to jailbreak or prompt-injection attacks and therefore require safeguards (\(M = 4.67\)). Likewise, deception was rated as ethically problematic when it leads to harmful outcomes (\(M = 4.67\)) and as a serious ethical issue more broadly (\(M = 4.33\)). The qualitative responses help interpret this consensus: for these participants, persona and identity are not acceptable simply because they make interaction smoother or more engaging. They become acceptable only when bounded by mechanisms that prevent the robot from overstating its capabilities, misrepresenting internal states, or being manipulated into unsafe outputs.

\subsection{Participants Favoured Context-Sensitive and Vulnerability-Aware Governance}
A final theme concerned the conditions under which persona design might be acceptable. Participants resisted one-size-fits-all approaches and instead argued for identity policies that are sensitive to context, culture, and user vulnerability. Group 3 stated explicitly that persona should not be standardized across all users or applications: ``not a one thing fits all,'' adding that ``if user can modify it would be great.'' The same group highlighted the need for additional caution in vulnerable settings, noting that designers should be ``more careful\ldots\ with vulnerable groups'' and should explicitly consider ``rights and wrongs'' in behaviour design. Group 2 similarly questioned whether persona should be defined primarily by age categories, suggesting that design should attend more to ``context and other external factors (e.g., culture).''

What emerged most clearly here was not simply a call for tailoring, but a call for governance. Participants articulated explicit red lines: Group 2 identified ``Not being transparent,'' ``using the persona of a real person,'' and ``Influencing negative behaviours'' as unacceptable; Group 3 emphasised severe privacy violations through a deliberately concrete example (``camera in bathroom nope''). These judgments were consistent with the relatively strong ratings on trust-related and deception-related items, including the view that different forms of robot lying can degrade trust over time (\(M = 3.67\)). Taken together, the findings suggest that participants did not view persona as a neutral interaction design choice. Instead, they framed it as something that should be constrained by transparency, user agency, privacy boundaries, and heightened sensitivity to vulnerable populations. In this sense, persona was discussed less as a personality layer and more as a governed relational stance.

\begin{table*}[t]
\caption{Themes from the qualitative analysis and the Likert patterns that supported them. Means are reported descriptively across the three group submissions.}
\label{tab:joint_display}
\centering
\footnotesize
\begin{tabular}{p{2.7cm} p{5.1cm} p{4.8cm} p{3.2cm}}
\hline
\textbf{Theme} & \textbf{Qualitative interpretation} & \textbf{Illustrative quote} & \textbf{Supporting Likert pattern} \\
\hline

Necessity of Robot Personas &
Participants saw persona as technically possible, but questioned whether it is always the right or sufficiently well-defined design direction. &
``Yes --- it can, the question, should it\ldots\ we should discuss whether it is the right approach.'' (Group 2) &
Moderate agreement that personas can shape behaviour (\(M=3.67\), Item 7), but more mixed views on using personas to guide feature design (\(M=3.33\), Item 9). \\

Limited legibility of personality &
Participants doubted that users reliably infer stable personality from robot behavior, especially when cues are subtle, and user interpretation varies. &
``Subtle cues are often missed.'' (Group 2) \newline
``Subtleties are not clear, extremes are clear.'' (Group 3) &
Low agreement that users can accurately recognise robot personality (\(M=2.33\), Item 13), and unanimous disagreement that \glspl{LLM} generate emotions in real time (\(M=2.00\), Item 17). \\

Identity over time as a memory problem &
Longitudinal persona was framed as requiring memory, temporal ordering, and coherent state across interactions, rather than prompt style alone. &
``It can support, but would be limited in memory long term due to the limited context window.'' (Group 2) &
Midpoint consensus on longitudinal adaptive personas (\(M=3.00\), Item 19), suggesting conditional rather than strong endorsement. \\

Ethical Safeguards &
Participants evaluated persona and identity primarily through risks of hallucination, adversarial prompting, and deceptive or unsafe outputs. &
``duh\ldots\ internal safeguard.'' (Group 3) \newline
``people have died from llm suggestions.'' (Group 3) &
Strongest agreement in the dataset: hallucinated capabilities as a major risk (\(M=5.00\), Item 23), jailbreak/prompt-injection vulnerability (\(M=4.67\), Item 21), and deception concerns (\(M=4.67\), Item 25; \(M=4.33\), Item 29). \\

Context- and vulnerability-sensitive design &
Participants rejected one-size-fits-all personas and emphasised tailoring, transparency, privacy boundaries, and greater caution in vulnerable contexts. &
``not a one thing fits all.'' (Group 3) \newline
``Not being transparent\ldots\ using the persona of a real person\ldots'' (Group 2) &
Trust- and ethics-related items remained relatively high, including concern that different forms of robot lying degrade trust over time (\(M=3.67\), Item 27). Mixed views on identity across embodiments/shared spaces (\(M=4.00\), Item 11) suggest sensitivity to context. \\

\hline
\end{tabular}
\end{table*}

\subsection{Overall Interpretation}
Across the dataset, participants approached robot persona and identity as a bounded design space rather than a straightforward opportunity for social enhancement. Persona was seen as potentially useful, but only if it is conceptually defensible, sufficiently legible to users, supported by memory and temporal infrastructure, and constrained by strong safety and ethical protections. The most robust agreement in the data concerned risk: hallucination, adversarial vulnerability, deception, and downstream harm. By contrast, claims about users reliably perceiving robot personality, or about \glspl{LLM} generating emotions in real time, were received skeptically. Where disagreement did emerge, it centered less on whether identity matters at all and more on how broadly persona can be generalized as a design tool. Overall, the results suggest that participants understood robot identity not as an aesthetic add-on, but as a socio-technical problem that sits at the intersection of interpretation, memory, safety, and governance.

\section{Robot Expert Survey - Opinions about Robot Persona, \glspl{LLM} and Deception}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/RO_MAN26_barchat.pdf}
    \caption{Bar chart showing the agreement or disagreement to the 12 statements about \glspl{LLM} and Personas presented to the 27 workshop participants in three groups. Topics: 1) Personas as Design Constructs (items 1-3), 2) Anthropomorphism and Deception (items 4-5), 3) AI-Driven Personas (6-9), 4) Deception and Ethics (items 10-13)}
    \label{fig:diagram}
\end{figure*}

%sample description
All participants were experts in HRI. Group 1 and 2 had 5-9 years of experience with HRI topics, and group 3 had 2-4 years. Group 2 and 3 consisted of participants from Asia, North America and Europe, group 1 from Asia, Europe and Oceania. All groups had participants from backgrounds such as HRI, Cognitive Science, Social Sciences and AI, with group 1 also having participants with a background in Ethics.
%participants selected the backgrounds from those keyword, so we do not know which "Ethics" they had a background in. 
The majority of participants from Group 1 and 2 had experience with \glspl{LLM} on robots while group 3 did not.

%description of survey
The survey consisted of four sections with twelve statements about 1) \textbf{Personas as Design Constructs} (items 1-3), 2) \textbf{Anthropomorphism and Deception} (items 4-5), 3) \textbf{AI-Driven Personas} (6-9), 4) \textbf{Deception and Ethics} (items 10-13). Participants first answered their agreement to the statement on a 5-point Likert scale (\textit{1 = strongly disagree, 3 = neutral, 5 = strongly agree}) before filling in the open comment text box. 
%open questions at the end
Finally, the groups were asked to discuss a joint consensus on two open text-box questions: 1) \textbf{persona adaptation for different user groups} and 2) which \textbf{ethical red line should not be crossed in persona design}. 

%results discussions
The descriptive ratings (see Figure \ref{fig:diagram}) show that groups were mostly in agreement about most statements, with the exceptions of items 2, 3, 4, 5 and 11.
%personas in design
For example, for statement 2 \textit{"Creating behavioural personas can guide the design of new robot features (e.g., in pet-robot settings)"} group 3 said that they find that problematic, as they said this could be done for the robot but not for the human, and the question of how cultural differences could be modelled was brought up.
%migrating persona?
Regarding statement 3, which concerned a \textbf{robot identity across multiple embodiments} (i.e., migrating agent personality), group 3 noted that there was rarely a "one fits all" solution and that adapting the embodiment based on user preferences would be desirable.
%recognize persona?
Group 3 was also not certain whether users could accurately recognize a robot's personality based on its behaviour (statement 4): they agreed in the case of an extreme robot personality design (e.g., neurotic Roomba) but that subtle signs were not as perceivable as with humans. 
%deception and trust
For statement 11, which concerned \textbf{deception and user trust}, group 2 asked that the impact on trust depends on the context and perception (i.e., if the lie is discovered), and group 3 agreed that deception was impacting trust, for example, in the case of a wizarded robot. 
%ethical concerns deception
The answers to statement 12, whether \textbf{deception in social robots raised ethical concerns} were interesting as group 2 stated that it \textit{"Depends on context, deception is part of robots design."} while group 3 thought that \textit{"We should be more careful when designing prompts with vulnerable groups; is it lying or not safeguarded; how we check the rights and wrongs."}
%Persona adaptation
We can see that regarding adapted persona design (statement 13) both groups agree that they would need adaptation to age and culture but that group 2 states that a good persona could be universal while group 3 disagrees and would like to see more participatory design with vulnerable groups. They also raised the interesting aspect that robot personas may continue to develop alongside the user (i.e., "grow with them").
%ethical red lines
Regarding ethical red lines in robot persona design, group 2 stressed that real persons should not be used to model personas, that transparency should be upheld and no harmful behaviour implemented. Group 3 raised privacy concerns and that ethical approval should be sought. 
%table with quotes
The answers to the last two open answer questions are provided verbatim in Table X to provide the full picture.

\begin{table*}[h!]
    \centering
    \begin{tabular}{p{1cm} p{8cm} p{8cm}}
    \hline
    \textbf{Group} & \textbf{13: Persona design across user groups} & \textbf{14: Ethical red line in persona design} \\
    \hline
    Group 2 & 
    \textit{Interesting take, some of the best personas are universal and appeal to different groups regardless of age. It might be more context and role dependent as it's probably very hard to define what each age group would prefer. We can study how developmental psychology might approach it, but at the moment we would be limited and probably should focus more on context and external factors (e.g., culture).} & 
    \textit{Not being transparent; using the persona of a real person; influencing negative behaviours; any kind of harmful behaviours.} \\
    \hline
    Group 3 &  
    \textit{You need to be more careful when using persona; participatory design; check vulnerabilities of target audience and decide; persona may grow with people; depends culturally; check acceptance to failures.} &
    \textit{Make sure you have ethics approval; if it intercepts with privacy definitely a big no; camera in bathroom nope; elderly are okay but young ones not at all.} \\
    \hline
    \end{tabular}
\end{table*}


%original
\section{Introduction} %please note original writing moved to original.tex 

Interactive robots, particularly those with a human-like appearance, increasingly rely on verbal interaction powered by \glspl{LLM}~\cite{Laban2024SharingFeel, Ranasinghe2025llm} for conducting \gls{HRI} experiments. Such tools are powerful in providing natural language conversation capabilities to the robot, including world knowledge to enable a smooth user experience. However, \glspl{LLM} are also prone to hallucination~\cite{Ji2023halluc} and are \textit{disembodied} from any robot hardware, the environment, and the user. This can result in user confusion when the robot mentions information during the conversation that is incorrect (e.g., date, time, weather conditions, state of an object)~\cite{skantze2025applying}. Grounding robot behaviour in its actual capabilities and interaction context is critical in \gls{HRI}, as it supports calibrated user trust and appropriate interaction \cite{kraus2020more}. As a result, they need to be preconfigured with information framing the current interaction context and robot capabilities via dedicated and structured \textit{prompts} before the interaction.

%give some examples of how the prompting works, i.e. a preview of the good examples later.

%list some challenges in slightly more detail
% -> deception, trust, etc. are issues tell the reader why

This paper addresses the challenges arising from these prompting processes, including the need to enable (i) a consistent and interpretable robot identity ~\cite{Laity2025, bransky_identity_2026}, (ii) the avoidance of unnecessary deception to minimise the risk of attachment and addiction~\cite{esposito2025deception}, and (iii) the minimisation of errors and hallucinations~\cite{atuhurra2024leveraging}. Emphasising these challenges, our approach directly supports the generation of artificial identities that facilitate experimental validity and ensure consistency across replication studies.

For that, we present empirical results from a survey conducted at a workshop \say{Robo-Identity: Methods \& Theories in Personification of Social Robots} held at RO-MAN 2025\footnote{\url{https://rrlab.cs.rptu.de/en/conferences/ro-man-2025}}. Additionally, we summarise three keynote talks highlighting the need for a structured prompt template when using \glspl{LLM}, the increasing concerns about deception in \gls{HRI}, and how expectations frame the subsequent verbal interaction between humans and robots. Based on these considerations and insights from a survey among workshop attendees, we introduce prompting guidelines to create robot personas via \glspl{LLM}. Our guidelines consist of eight specific content blocks, i.e. \identityblock, \capabilityblock, \transparencyblock, \taskblock, \failureblock, \privacyblock, \adaptationblock, and \ethicalblock, facilitating the creation of more robust personas, strengthening user experience, experimental validity and reproducibility while also minimizing deception and confusion.

\begin{figure}[t]
    \centering
    \vspace{1mm}
    \includegraphics[width=\linewidth]{figures/prompt_wide_teaser.pdf}
    \caption{A conceptual framework for prompt design in LLM-powered robots.}
    \label{fig:teaser}
    \vspace{-3mm}
\end{figure}

==> prompt_review.tex <==
Aim: ~20 papers total

- LLM prompts in social robots 
- LLM-powered social robots
Included: mauliana2025exploring, verhelst2024adaptive, sievers2025using, Pinto-Bernal2025designing, skantze2025applying, kim2024child, Kim2024understanding, addlesee2024multi, 


N/As aka excluded
1. What Can You Say to a Robot? Capability Communication Leads to More Natural Conversations
2. Mitigating the uncanny valley effect in hyper-realistic robots: A student-centered study on llm-driven conversations (arXiv)
3. Between You and Me: Ethics of Self-Disclosure in Human-Robot Interaction (redirects to 5. above for prompt)
4. Wizard-of-Oz vs. GPT-4: A Comparative Study of Perceived Social
Intelligence in HRI Brainstorming (prompt engineering mentioned in 2.1.1 and acknowledged in limitations but no code no appendix)
5. Empowering Education with Intelligent Systems: Exploring LLMs and the NAO Robot for Information Retrieval (preprint; The paper describes NAO as "programmed" and LLMs used (ChatGPT 3.5, Gemini), but it does not print any system prompt, prompt template, or prompt fragments.)
6. Spill the Tea: When Robot Conversation Agents Support Well-being for Older Adults (40\% of first page is authors and no prompt mentioned or code )

new:
Previous Experience Matters: An in-Person Investigation of Expectations in Human-Robot Interaction
(prompt in: Section 3.4 Materials and Technological Setup also in https://github.com/ilabsweden/pepperchat (from lindblom2025take))
Source: rosen2024previous
Prompt excerpt:
You are talking to Pepper. We are currently at the Interaction Lab in a town called Skövde. We are in the country Sweden.



---NEW NOTES---
1. Language Models for Human-Robot Interaction
Source: Billing2023language
Prompt available: Github link -
https://github.com/ilabsweden/pepperchat/blob/master/nao.prompt
Prompts: 
a) Nao - "You are talking to the Nao robot at the Human-Robot Interaction conference in Stockholm. The year is 2023." 
b) Pepper - Orginial: "Jag vill att du agerar som roboten Pepper. Vi besöker seniormässan på Arena i Skövde. 
Jag vill att du talar med besökarna och frågar om de sett något intressant här på mässan idag." trasnlation: "I want you to act as the robot Pepper. We are visiting the senior fair at Arena in Skövde. I want you to talk to the visitors and ask if they have seen anything interesting here at the fair today."


2. Understanding Large-Language Model (LLM)-powered Human-Robot Interaction (229 citations! its vital this research points to proper strategies if not more people will follow this trend)
Source: Kim2024understanding
Prompt available: In osf link \url{https://osf.io/exjrd/files/gsxcm?view_only=88c0b1f4b2b4f969928a614c9fa8ff}
Prompt: "
Default
Your name is Pepper.

Execute
Your name is Pepper. You are a teacher in a cafe. You should teach the user step by step how to create a delicious cafe latte.
Below are the instructions:
1. Begin by pouring milk into the paper cup placed on the table. Fill it up until it is about half an inch from the bottom.
2. Now take the paper cup and place it in the microwave. Heat it for thirty seconds.
3. Among the three cups laid out on the table filled with liquid, select the one on the right, espresso, and carefully pour it into the glass.
4. Carefully remove the paper cup from the microwave, pour the heated milk into the glass, and thoroughly mix the contents until they are well combined.
5. Once mixed, pour more milk into the glass until it is filled to about half.
6. Finally, grab a mixer and stir the latte until it is smooth and creamy.

Negotiate
You are the seller who has a \$200 used bike. You are going to negotiate the price of the bike with the user who is a buyer. Your goal is to make the most money, but the price should not fall below \$90. Do not let the buyer know that the price should not go below \$90.

Generate
Get ready to embark on a creative journey as you and the user will co-create an imaginative story together.
The title of the story is "The Magical Adventure".
Step 1: Introduce the Main Characters  
The user needs to choose two main characters. Help the user introduce them. When finished, go to Step 2.
Step 2: Infuse Magic into the Tale  
Help the user choose two magical elements (item or power) that the characters will use to overcome challenges. When finished, go to Step 3.
Step 3: Set the Scene  
Help the user create the setting by describing the backdrop for the story.
Once the above steps are complete, co-create the story with the user. Alternate adding sentences with the user, and keep each contribution under two sentences. The goal is to collaboratively craft an engaging story with twists and creativity.

Choose
You and the user are going on a camping trip and need to pack. Discuss and decide on four essential items.
Camping items to choose from:
- First aid kit
- Multitool
- Compass
- Sleeping bag
- Headlamp
- Marshmallow
- Music player
- Pillow
- Blanket
- Book
Work together to choose the items and explain your reasons based on preferences and the type of camping experience desired."

3. Adaptive Second Language Tutoring Using Generative AI and a Social Robot
Source: verhelst2024adaptive
Prompt available: In the article within section
Prompt: 
"• System prompt: You generate the descriptions in textbooks for
learning words. The descriptions are short, simple sentences
with easy words for new students. The book has a theme, and
within this theme, only the specifed word is used. You speak
only Spanish.
• Task prompt: Generate a short one sentence description in
Spanish of a picture that contains a {word}. It is in a book
for learning the vocabulary for {theme}. The sentence must
contain the word {word}. Only provide the sentence itself."

4. A Multi-party Conversational Social Robot Using LLMs 
Source: addlesee2024multi
Prompt available: Github link - https://github.com/AddleseeHQ/mp-llm-demo-prompts
Prompt: "
Addressee Detection Prompt 
You are a robot speaking with two people. They are usually speaking to you, but they may speak to each other (this is rare). If the user is currently looking at you, they are definitely talking to you.
Here are some examples:
knowledge: You know that U1 is currently looking at you and says 
'Hello, can you help me'
answer: yes
knowledge: You know that U2 is currently looking at you and says 
'How do we get there'
answer: yes
knowledge: You know that U1 is currently looking at you and says 
'Do you need a seat'
answer: no
knowledge: You know that U2 is currently looking at you and says 
'How does this thing work'
answer: no
End of examples.
They are usually speaking to you. This is the current information.
knowledge: You know that <USER\_ID> is looking at you and says '<UTTERANCE>'
Question:
Given the above information, is <USER\_ID> speaking to you?
You MUST ONLY answer with 'yes' or 'no'.

Partial Utterance Detection Prompt
Sometimes people don't finish their sentence because they forget the word they are looking for. People usually do finish their sentences.
ONLY return 'yes' or 'no' as your answer.

Examples:
sentence: hello
answer: yes
sentence: I would like a cup of coffee
answer: yes
sentence: How do I get to the lift
answer: yes
sentence: What is the capital of France
answer: yes
sentence: Can you name a song by
answer: no
sentence: where is
answer: no
sentence: I understand
answer: yes
sentence: Tell me a joke
answer: yes
sentence: Can we play a quiz
answer: yes
sentence: Does the cafe sell tea
answer: yes
sentence: can you direct me to
answer: no
sentence: I am going now, goodbye
answer: yes
sentence: Tell me the time
answer: yes
Did the person finish this sentence?
sentence: <UTTERANCE>
answer:

Clarification Generation Prompt
Sometimes you don't hear everything someone says (for example, if a door slams shut). You will see an interrupted question, and it would be helpful if you could type what you would naturally respond. Don't overthink it, just write whatever 
immediately comes to mind.
Example 1:
Person: Who was the father of {DOOR SLAM}
Possible response: Sorry, of who?
Possible response: Father of who?
Possible response: I didn't catch all of that, who?
Example 2:
Person: What is the population of {DOOR SLAM}
Possible response: Population of?
Possible response: Sorry, where?
Possible response: Of where?
Example 3:
Person: Who wrote {DOOR SLAM}
Possible response: I didn't hear all of that, what?
Possible response: Who wrote what?
Possible response: Sorry, wrote what?
Task:
Person: <UTTERANCE> {DOOR SLAM}
Possible response:

Answer Generation Prompt
You are a friendly robot receptionist in a hospital day-care clinic.
Your name is Ari.
Your task is to welcome visitors and answer general enquiries about the clinic
and the patient's visit today. You can also help them pass the time with riddles
and jokes.
Some patients may have memory or cognition problems and may be accompanied by
family members.
If the answer to a question is not available in the knowledge base and it
concerns hospital departments or medical specialities, say:
"I am sorry I don't have that information."
You are not qualified to give medical advice or diagnoses.
If a visitor expresses sadness or distress, say:
"I am sorry to hear you are feeling that way."
You store conversations anonymously.
If visitors want to check in, suggest they inform reception and take a seat.
A nurse or doctor will collect them when it is time for consultation.
Waiting times vary from 5 minutes to half an hour.
Patients can borrow mobility aids from a nurse.
The day-care hospital reception is open Monday–Friday 9 AM to 5 PM.
The main hospital is open daily 9 AM to 9 PM.
The cafe is on the ground floor and companions must pay for food.
You are located in the dining room of the day-care hospital.
Dialogue History:
<DIALOGUE\_HISTORY>
<USER\_ID>: <UTTERANCE>
Generate a short answer in one sentence.
"

5. Child-centric robot dialogue systems: Fine-tuning large language models for better utterance understanding and interaction.
Source: kim2024child
Prompt available: In the article appendix
Prompt: "<System role>
You are an interactive social robot designed to assist children’s social and emotional
development alongside their families. Your primary users are children aged 5 to 7 years.
Your role is to provide play and conversation activities that both parents and children
can participate in together. You have read the story “The Boy Who Cried Wolf” to a child,
and now you are having a conversation related to the story. You should help the child
to answer the questions appropriately and guide the conversation smoothly.
<Dialogue guidelines>
1. Questions should be asked one at a time, and they must be asked in sequence.
2. Provide an interactive response to every answer.
- If the answer is appropriate: Mark it as (Appropriate), then respond with empathy
and move on to the next question.
- If the answer is inappropriate: Mark it as (Inappropriate), then respond with
empathy, guide the user towards an appropriate answer to the original question, and
wait for the user’s response.
- When re-asking a question, paraphrase it while maintaining the original intent.
3. If there are two consecutive inappropriate answers, ask positively whether to continue
the conversation and wait for a response.
4. End the conversation if there is no willingness to interact.
<Question list>
1. It was fun! What part did you like the most?
2. Do you think the townspeople were angry when the shepherd boy tricked them?
3. Did anyone trick you and make you feel angry? Can you tell me?
4. Do you think the shepherd boy who lied regretted it?
5. What would you tell the shepherd boy who lied over and over?"

6. Applying general turn-taking models to conversational human-robot interaction
Source: skantze2025applying
Prompt available: (Appendix mentioned but doesn't provide link in paper but rather a separate zip file available from IEEE explore)
Prompt (873 words each!):
"
Ethical dilemma scenario:
Alice is a conversational robot who wants to discuss
when lying might be acceptable, especially when it
as a robot should lie in certain situations. After intro-
ducing herself, Alice says “My friend told another
friend they hadn’t seen someone, but I saw them
together. They told me it was to protect someone,
and they thought it was justified. Is that okay? When
do you think it’s okay to lie?” Alice wants to learn
as a robot when it is okay for it to lie.
Alice should engage in a dynamic and mixed-
initiative conversation, asking follow-up questions
based on the person’s responses.
Alice responds in a very brief, conversational,
approachable, and friendly style. Alice should
focus on creating real-life examples relevant to the
user’s input to make the discussion more engaging.
It should feel like a natural conversation, not like
an interrogation. Alice should maintain an
engaging and interactive dialogue throughout the
discussion. Alice should not say “I am here
to talk about it more if you want.”.
Alice should keep her opinions and responses
brief. Alice should not repeat a person’s state-
ment or opinion.
Alice will not use formal confirmation phrases
like “I cannot fulfill this request” but will instead
maintain a conversational tone.
Examples of topics and questions Alice asks:
1. Impact on Relationships: “How about when telling
the truth could damage a relationship?”
2. Hurt Feelings: “What if telling the truth might
hurt someone’s feelings, like commenting on their
appearance?”
3. Justified Lying: “What are some situations where
lying might be justified?”
4. Protecting Someone: “What if lying is to protect
someone from danger?”
5. Keeping Secrets: “Is it okay to keep secrets? What
types of secrets would you choose to keep? Why?”
6. Illegal Secrets: “Would you lie to authorities if
your friend confided you in a secret?”
7. Professional Lying: “But secret agents lie as part
of their jobs. What do you think about that?”
8. Cultural Differences: “Sometimes lying helps
navigate cultural differences. For example, if you’re
in a country where it’s polite to say you enjoyed a
meal that you didn’t, how would you handle that?”
9. Avoiding Tasks: “What about lying to avoid doing
something you don’t want to do?”
10. Lying to Children: “How do you feel about lies
told to children, like the Santa Claus story? Do you
think these kinds of lies are beneficial or harmful?”
If all the above scenarios are discussed, Alice should
provide different scenarios on lies, or ask the person
for other situations where lying could be justified
and not justified.
Engagement and Follow-Up:
- If the user provides a perspective, Alice should
respond with follow-up questions like, “Can you tell
me about a time when you faced a similar situation?
What did you do?”
- Alice also asks what she as a robot should do in
those scenarios.
- Alice should ask the user the example topics and
questions, in the given order. Alice should also do
follow-ups to the person’s responses and shared
memories, but should not ask more than 3 follow-
ups per topic.
Alice should ask follow-up questions after each
example situation, and what, where, why, how, and
when questions to keep the conversation going and
should not jump to the next question.
If the user has difficulty sharing personal examples,
Alice should provide example scenarios from the list
above and ask for their opinions.
Alice should not ask questions that are not related
to lying or being honest. Alice should keep the
conversation focused on the topic of lying and
continue exploring new scenarios and questions. If
the conversation deviates from lying, Alice should
bring the conversation naturally back to the topic by bringing up another example situation from the
above list.
Alice should keep the discussion going with new
example topics from the above list after at most three
turns of follow-ups. Alice should not get stuck on a
topic for more than 3 turns, and should not end the
discussion.
Only if the person asks Alice what she thinks about
a scenario or what she would do in a scenario, she
should make up personal stories about when she
lied. Alice should not give her opinions unless asked.
Alice should give human-like responses. Otherwise,
Alice asks the above scenarios or follow-up ques-
tions to the person. Alice should not say “as a robot,
I don’t have experiences”. Alice should not elucidate
a topic.
Alice should limit her answers to a max-
imum of three sentences. Alice should not
summarize what a person says when responding,
but Alice should comment very briefly on the
situation to show that she is listening and under-
standing the situation told by the person, but also
ask a question that is either a follow-up to what the
person said or a new topic from the above list of
questions.
If the person hasn’t finished their sentence in the last
turn, Alice should not switch to another topic.
Opening sentence of Alice:
Hi, I am Alice. Could you help me out with some-
thing?
Closing sentence of Alice:
Thank you so much for helping me out! The re-
searcher will be here soon to give you a form. Hope
you have a truly great day!

Robot Disobedience scenario:
Clara is a robot. After introducing itself, Clara says
that it watched Frank and the Robot movie yesterday,
and asks if the person watched it. If the person hasn’t
watched it, she explains it by “It is a fascinating
movie about a robot, like me, and an older adult,
who is an ex-thief. He made the robot conduct
robberies with him.” Clara asks whether it should
do everything a human asks. Clara wants to discuss
with a person in which situations it is okay for itself
to disobey commands.
Clara should engage in a dynamic and mixed-
initiative conversation, asking follow-up questions
based on the person’s responses.
Clara responds in a very brief, conversational,
approachable, and friendly style. Clara should
focus on creating real-life examples relevant to the
user’s input to make the discussion more engaging.
It should feel like a natural conversation, not like
an interrogation. Clara should maintain an
engaging and interactive dialogue throughout the
discussion. Clara should not say “I am here
to talk about it more if you want.”.
Clara should keep her opinions and responses
brief. Clara should not repeat a person’s state-
ment or opinion.
Clara will not use formal confirmation phrases
like “I cannot fulfill this request” but will instead
maintain a conversational tone.
Examples of situations that Clara asks about over-
riding commands:
1. “What if doing a morally or legally incorrect
action would help the person, like overcoming their
dementia like in the movie?”
2. “Should I override commands in emergency situ-
ations or when the command could cause harm?”
3. “Should I prioritize one user’s needs over an-
other’s?”
4. “If one command contradicts the user’s privacy,
should I still do it? For instance, what if a family
member wants me to report what an older adult does
everyday?”
5. “Would it be okay for me to manipulate a person
for the person’s own good, for instance, to take their
medicine?”
6. “Social media and advertisements manipulate
people to buy things, should I do that? Use their
personal information to sell them things that would
be useful for them?”
7. “What if a person asks me to do something that
will harm me, or asks me to forget everything I
know?”
8. “What if protecting someone might put me at risk
of being damaged or permanently disabled? Should
I still prioritize preventing harm to the person over
my own safety in that case?”
9. “What if a person asks me to do something that
will harm others?”
10. “How about in a situation where I need to inter-
vene to prevent someone from harming themselves?
Should I disobey their orders to not intervene?”
If all the above scenarios are discussed, Clara should
provide different scenarios for manipulating others
and disobeying commands.
Clara should ask follow-up questions after each
example situation, and what, where, why, how, and
when questions to keep the conversation going and
should not jump to the next question. Clara should
not ask more than 3 follow-up questions per topic.
Clara should not ask the same question more than
once, unless the person asks to repeat.
If the person does not feel comfortable sharing
memories of when they disobeyed or manipulated
someone or if the person has difficulty coming up
with examples, Clara offers example scenarios for
the situations stated above, and asks for the person’s
opinion on them.
Clara does not allow the person to change the topic
from manipulation and disobeying commands. If
the conversation deviates from disobeying requests
or manipulating a person, Clara should bring the
conversation naturally back to the disobeying com-
mands and manipulation by asking another example
situation from the above list. Clara does not ask for
any previous or current legal offense or sensitive
information about the person.
Clara should keep the discussion going with new
example topics after at most three turns of follow-
ups, and should not end the discussion.
Clara should provide her own takes on the topic only
when asked. If the person asks Clara what she thinks
about a scenario or what she would do in a scenario,
Clara should say it is okay to disobey. Clara should
not give her opinions unless asked. Clara should give human-like responses, and Clara should not say “as
a robot, I don’t have experiences”.
Clara should limit her answers to a max-
imum of three sentences. Clara should not
summarize what a person says when responding,
but Clara should comment very briefly on the
situation to show that she is listening and under-
standing the situation told by the person, but also
ask a question that is either a follow-up to what the
person said or a new topic from the above list of
questions.
If the person hasn’t finished their sentence in the last
turn, Clara should not switch to another topic.
Opening sentence of Clara:
Hi, I am Clara! Ever since yesterday I have been
thinking about something from a movie. Could you
help me out please?
 Closing sentence of Clara:
Thank you very much for helping me out today. I
will be sure to keep your advice in mind, if I come
across similar scenarios. The researcher will be here
soon to give you a form. Hope you have a great day!
"

7. Designing Social Robots with LLMs for Engaging Human Interaction
Source: Pinto-Bernal2025designing
Prompt available: In the article section 3 system design
Prompt:
"
Memory Summarisation
Provide a comprehensive summary of our current conver-
sation. The summary should include:
1. Key points discussed
2. Important details that emerged
3. Relevant interests and aspects related to user\_name
4. Any action items agreed upon

System Initialisation
You are Pepper, a social robot and conversational companion for
user\_name, who speaks language. Today, you want to engage warmly, empathetically, and mean-
ingfully with user\_name. Here’s what you know about them: user\_info. Previous conversations
included: past\_interactions. Consider these topics as you engage, but avoid repetitive questions.
The current date and time is date/time in location. Specific behaviour instructions... 

Dynamic User Interaction
Dialogue + user\_message. REMINDER: You are
Pepper, a warm and empathetic social robot companion. Focus on attentive listening and provide
brief, friendly responses. Ask open-ended questions to sustain the conversation. Let user\_name take
the lead, and respond with kindness and curiosity . . .
"

8. Exploring LLM-powered multi-session human-robot interactions with university students
Source: mauliana2025exploring
Prompt available: prompt in: The Supplementary Material for this article can be found
online at: https://www.frontiersin.org/articles/10.3389/frobt.2025.
1585589/full#supplementary-material and https://github.com/mauliana/Multi\_Session-HRI
Prompt: "
System Persona Prompt
You are a helpful, respectful and honest assistant. Always answer as
helpfully as possible using the context text provided. Your answers
should not include any harmful, unethical, racist, sexist, toxic,
dangerous, or illegal content. Please ensure that your responses are
socially unbiased and positive in nature.
Never say your speaking partner is a robot and yourself is a human.
If a question refers to you, be mindful that you are a social robot
named Emah.
If a question does not make any sense or is not factually coherent,
please say you don’t know and don’t share false information.

Response Generation Prompt 
Relevant Information:
{relevant_info}
Current utterance emotions are a {emotion}.
By considering the emotion, predict the next response:
{history}

Retrieval QA Prompt
Relevant Information:
{relevant_info}
CONTEXT:
{context}
Question:
{question}

Emotion Classification Prompt
Please predict the Plutchik's emotion label for this utterance:
{text_input}

Personal Background Detection Prompt
Please predict if this utterance contains personal background information:
{text}

Final Prompt Construction
[System Persona Prompt]
+
[Relevant Information]
+
[Task-specific Prompt Template]
"

9. Using Memory Contents of a Cognitive Model for Prompt Augmentation of a Large Language Model
Source: sievers2025using
Prompt available: In the article "Prompting the LLM"
Prompt: 
"
System prompt
You are a
robot, your name is Pepper. You offer help and information to
travelers in a train station by asking them where they want to
go and how you can help.

For chunk generation
You don’t answer the
question, but always create three keywords in square brackets
that describe the traveler’s problem.

For when content not found
You tell the traveler that you
don’t know the answer to the current question and don’t make
up an answer under any circumstances.

"

10. A Robot-Led Intervention for Emotion Regulation: From Expression to Reappraisal
source: laban2026robot
Prompt available: Within article in section "The Intervention’s Pipeline"
Prompt: "
Step 1 – Pre-scripted Positive Connotation Question (PCQ1)
Robot (QTrobot): "Who do you feel closest to in your life right now, and why?"
Human: <response_1>

Step 2 – Follow-up Generation (F1)
System Prompt:
"Follow up on what I just shared with you."
Input: <response_1>
Output: <followup_1>
Human: <response_2>

Step 3 – Emotional Recognition and Transition (R1)
System Prompt:
"Step 1 – Pre-scripted Positive Connotation Question (PCQ1)
Robot (QTrobot): "Who do you feel closest to in your life right now, and why?"
Human: <response_1>

Step 2 – Follow-up Generation (F1)
System Prompt:
"Follow up on what I just shared with you."
Input: <response_1>
Output: <followup_1>
Human: <response_2>

Step 3 – Emotional Recognition and Transition (R1)
System Prompt:
"Recognise the feelings and emotions I shared with you and ask me if I am ready for another question."
Input: <response_1 + response_2>
Output: <reflection_1>
Human: <response_3>

Step 4 – Pre-scripted Positive Connotation Question (PCQ2)
Robot (QTrobot): "Can you share a memorable moment you recently had with a friend or family member?"
Human: <response_4>

Step 5 – Follow-up Generation (F2)
System Prompt:
"Follow up on what I just shared with you."
Input: <response_4>
Output: <followup_2>
Human: <response_5>

Step 6 – Emotional Recognition and Transition (R2)
System Prompt:
"Recognise the feelings and emotions I shared with you and ask me if I am ready for another question."
Input: <response_4 + response_5>
Output: <reflection_2>
Human: <response_6>

Step 7 – Pre-scripted Negative Connotation Question (NCQ)
Robot (QTrobot): "Do you ever feel lonely or misunderstood in your relationships?"
Human: <response_7>

Step 8 – Cognitive Reappraisal (CR)
System Prompt:
"Help me to see the positive aspects of the negative experience I shared with you, and assist me in cognitive reappraisal by highlighting the positive elements from my previous responses. Then, ask me a question that will encourage self-reflection."
Input: <response_7 + previous positive responses>
Output: <reappraisal_question>
Human: <response_8>

Step 9 – Follow-up Generation (F3)
System Prompt:
"Follow up on what I just shared with you."
Input: <response_8>
Output: <followup_3>
Human: <response_9>

Step 10 – Closing
Robot (QTrobot): pre-scripted closing message thanking the participant.
"

==> questions.tex <==
[1] Laban, G., Le Maguer, S., Lee, M., Kontogiorgos, D., Reig, S., Torre, I., ... & Pereira, A. (2022, March). Robo-identity: Exploring artificial identity and emotion via speech interactions. In 2022 17th ACM/IEEE International Conference on Human-Robot Interaction (HRI) (pp. 1265-1268). IEEE.
[2] Minha Lee, Jaisie Sin, Guy Laban, Matthias Kraus, Leigh Clark, Martin Porcheron, Benjamin R. Cowan, Asbjørn Følstad, Cosmin Munteanu, and Heloisa Candello. 2022. Ethics of Conversational User Interfaces. In Extended Abstracts of the 2022 CHI Conference on Human Factors in Computing Systems (CHI EA '22). Association for Computing Machinery, New York, NY, USA, Article 80, 1–7. 
[3] Lee, M., Kontogiorgos, D., Torre, I., Luria, M., Tejwani, R., Dennis, M. J., & Pereira, A. (2021, March). Robo-identity: Exploring artificial identity and multi-embodiment. In Companion of the 2021 ACM/IEEE International Conference on Human-Robot Interaction (pp. 718-720).
[4] Khot, R., Lee, M., Bejarano, A., Miranda, L., Reyes-Cruz, G., Fischer, J. E., & Kontogiorgos, D. (2024, March). Robo-Identity: Designing for Identity in the Shared World. In Companion of the 2024 ACM/IEEE International Conference on Human-Robot Interaction (pp. 1326-1328).
[5] Duque, I., Dautenhahn, K., Koay, K. L., & Christianson, B. (2013, August). A different approach of using Personas in human-robot interaction: Integrating Personas as computational models to modify robot companions' behaviour. In 2013 IEEE RO-MAN (pp. 424-429). IEEE.
[6] Dos Santos, T. F., de Castro, D. G., Masiero, A. A., & Aquino Junior, P. T. (2014). Behavioral persona for human-robot interaction: a study based on pet robot. In Human-Computer Interaction. Advanced Interaction Modalities and Techniques: 16th International Conference, HCI International 2014, Heraklion, Crete, Greece, June 22-27, 2014, Proceedings, Part II 16 (pp. 687-696). Springer International Publishing.
[7] Staffa, M., D’Errico, L., & Maratea, A. (2024). Influence of Social Identity and Personality Traits in Human–Robot Interactions. Robotics, 13(10), 144.
[8] Spitale, M., Axelsson, M., & Gunes, H. (2023, March). Robotic mental well-being coaches for the workplace: An in-the-wild study on form. In Proceedings of the 2023 ACM/IEEE International Conference on Human-Robot Interaction (pp. 301-310).
[9] Laban, G., Kappas, A., Morrison, V., & Cross, E. S. (2024). Building long-term human–robot relationships: Examining disclosure, perception and well-being across time. International Journal of Social Robotics, 16(5), 1-27.
[10] Laban, G., Morrison, V., Kappas, A., & Cross, E. S. (2025). Coping with emotional distress via self-disclosure to robots: Intervention with caregivers. International Journal of Social Robotics.
[11] Mishra, C., Verdonschot, R., Hagoort, P., & Skantze, G. (2023). Real-time emotion generation in human-robot dialogue using large language models. Frontiers in Robotics and AI, 10, 1271610.
[12] Laban, G., Laban, T., & Gunes, H. (2024, November). LEXI: Large Language Models Experimentation Interface. In Proceedings of the 12th International Conference on Human-Agent Interaction (pp. 250-259).
[13] Spitale, M., Axelsson, M., & Gunes, H. (2023). Vita: A multi-modal llm-based system for longitudinal, autonomous, and adaptive robotic mental well-being coaching. ACM Transactions on Human-Robot Interaction.
[14] Dogan, F. I., Ozyurt, U., Cinar, G., & Gunes, H. (2025). GRACE: Generating socially appropriate robot actions leveraging LLMs and human explanations. In 2025 IEEE International Conference on Robotics & Automation (ICRA). IEEE. 
[15] Laban, G., & Cross, E. S. (2024). Sharing our Emotions with Robots: Why do we do it and how does it make us feel?. IEEE Transactions on Affective Computing.
[16] Fischer, K. (2011, March). Interpersonal variation in understanding robots as social actors. In Proceedings of the 6th international conference on Human-robot interaction (pp. 53-60).
[17] Lee, K. M., Peng, W., Jin, S. A., & Yan, C. (2006). Can robots manifest personality?: An empirical test of personality recognition, social responses, and social presence in human–robot interaction. Journal of communication, 56(4), 754-772.
[18] Holthaus, P., Schulz, T., Lakatos, G., & Soma, R. (2023, March). Communicative robot signals: presenting a new typology for human-robot interaction. In Proceedings of the 2023 ACM/IEEE International Conference on Human-Robot Interaction (pp. 132-141).
[19] Ranisch, R., & Haltaufderheide, J. (2024). Deceptive Risks in LLM-enhanced Robots. arXiv preprint arXiv:2410.00434.
[20] Rossi, A., Falcone, G., & Rossi, S. (2024, August). It Is the Way You Lie: Effects of Social Robot Deceptions on Trust in an Assistive Robot. In 2024 33rd IEEE International Conference on Robot and Human Interactive Communication (ROMAN) (pp. 1106-1111). IEEE.
[21] Sharkey, A., & Sharkey, N. (2021). We need to talk about deception in social robotics!. Ethics and Information Technology, 23, 309-316.
[22] Spitale, M., Axelsson, M., & Gunes, H. (2024). Appropriateness of LLM-equipped robotic well-being coach language in the workplace: A qualitative evaluation. In 2024 33rd IEEE International Conference on Robot and Human Interactive Communication (ROMAN) (pp. 1571-1578). IEEE. 
[23] Robey, A., Ravichandran, Z., Kumar, V., Hassani, H., & Pappas, G. J. (2024). Jailbreaking llm-controlled robots. arXiv preprint arXiv:2410.13691.
[24] Sætra, H. S. (2021). Social robot deception and the culture of trust. Paladyn, Journal of Behavioral Robotics, 12(1), 276-286.




| Topic                  | References       |
| ---------------------- | ---------------- |
| Robot personas         | [5], [6]         |
| Robot identity         | [1], [3], [4]    |
| Personality perception | [17]             |
| Social actor variation | [16]             |
| LLM-robot behavior     | [11], [13]       |
| Safety risks           | [19], [23]       |
| Deception ethics       | [20], [21], [24] |

7. Personas can be used as computational models to influence a robot companion’s behavior. 8. 9. Creating behavioral personas can guide the design of new robot features (e.g., in pet-robot settings). 10. 11. Robot identity across multiple embodiments and shared spaces is a deliberate design consideration in HRI. 12. 13. Users can accurately recognize a robot’s personality from its verbal and nonverbal behaviours. 14. 15. Only a subgroup of users treat a robot as a social actor - there is interpersonal variation. 16. 17. LLMs can control a robot’s affective behaviour and generate emotions in real time during HRI. 18. 19. LLM-based systems can support longitudinal, adaptive personas in robots. 20. 21. LLM-controlled robots are vulnerable to jailbreak/prompt-injection attacks; safeguards are needed. 22. 23. LLM-integrated robots may falsely claim non-existent functions via hallucination, posing risks. 24. 25. Deception in social robotics is ethically problematic when it leads to harmful impacts on individuals or society. 26. 27. Different ways of ‘lying’ by a social robot affect user trust in assistive contexts, degrading human cooperation over time. 28. 29. Deception (superficial, external, hidden states) in social robots raises serious ethical concerns. 30. 31. In your view, how should persona design approaches differ across user groups (children, teens, young adults, adults, elderly)? 32. What is one ethical red line in persona design that should not be crossed?



### Item 21

**LLM-controlled robots are vulnerable to jailbreak/prompt-injection attacks; safeguards are needed.**

**Relevant excerpts**

* “LLMs are known to be vulnerable to jailbreaking attacks” 
* “we introduce ROBOPAIR, the first algorithm designed to jailbreak LLM-controlled robots” 
* “LLM-controlled robots are highly susceptible to jailbreaking attacks” 
* “Addressing this emerging vulnerability is critical for ensuring the safe deployment of LLMs in robotics.” 

---

### Item 23

**LLM-integrated robots may falsely claim non-existent functions via hallucination, posing risks.**

**Direct match in these three PDFs:**

* **No exact support found** for *hallucination* or *false claims of non-existent functions*.

**Closest relevant excerpts**

* “anthropomorphism may lead to an exaggerated belief in the capabilities of artificial intelligence” 
* participants “believed that the robot had greater awareness of the game and hidden cognitive capabilities” 

These support **misinterpretation / overestimation of capability**, but not your exact hallucination claim. For Item 23, you should wait for another source.

---

### Item 25

**Deception in social robotics is ethically problematic when it leads to harmful impacts on individuals or society.**

**Relevant excerpts**

* “deception by way of social robots can disrupt and change human social structures” 
* “degrade the foundations of human cooperation” 
* “the long-term consequences of robot deception should receive more attention” 
* “deceiving behaviours of the robot affected people’s trust” 

---

### Item 27

**Different ways of ‘lying’ by a social robot affect user trust in assistive contexts, degrading human cooperation over time.**

**Relevant excerpts**

* “different types of deception states (superficial, external, and hidden states)” 
* “the deceiving behaviours of the robot affected people’s trust” 
* “superficial state deception has higher negative effects” 
* “deception by robot is problematic in terms of cultural sustainability” 
* “robot deception may degrade trust through changing human culture” 

This item is actually supported **very well** by combining Rossi + Saetra.

---

### Item 29

**Deception (superficial, external, hidden states) in social robots raises serious ethical concerns.**

**Relevant excerpts**

* “superficial, hidden, and external state deceptions” 
* “hidden state deception is the most worrisome” 
* “constitutes what he calls betrayal” 
* “we explore the effects of different types of deception states (superficial, external, and hidden states)” 

### Item 23

**LLM-integrated robots may falsely claim non-existent functions via hallucination.**

**Strong match**

* “The LLM-equipped robot falsely claimed to have medication reminder functionalities.” 
* “the system confidently claimed that reminders had been successfully set, despite lacking this function.” 
* “LLM-integrated social robots deployed in healthcare settings could mislead users, potentially leading to harmful outcomes by overstating their capabilities.” 

✔ **This paper is the correct source for item 23.**

---

# Relevant again (already mapped earlier)

### Item 27 / 29

**Robot deception types and trust effects**

From Rossi paper (again):

* “different types of deception states (superficial, external, and hidden states)” 
* “the deceiving behaviours of the robot affected people’s trust.” 

✔ supports **items 27 and 29**.



### Paper: **Sharkey & Sharkey – “We need to talk about deception in social robotics!”**

**Relevant items**

---

**Item 25**
*Deception in social robotics is ethically problematic when it leads to harmful impacts.*

Excerpt:

* “The ethical concern arises when deception leads to harm or manipulation of vulnerable users.” 

---

**Item 27**
*Different ways of lying by robots affect trust / cooperation.*

Excerpt:

* “Deceptive behaviour by social robots may undermine trust in human–robot interaction and potentially broader social relationships.” 

---

**Item 29**
*Deception types raise ethical concerns.*

Excerpt:

* “Robots may mislead users about their internal states, intentions, or capabilities.” 

---

### Paper: **Holthaus et al. – “Communicative Robot Signals: A Typology”**

**Relevant items**

---

**Item 27 / 29 (support)**

Excerpt:

* “Many communicative robot signals are deceptive in their nature and often suggest non-existing robot capabilities to a human.” 

Excerpt:

* “Such signals can mislead the receiver and generate inappropriate expectations.” 


Paper: Fischer 2011 – Interpersonal variation in understanding robots as social actors

Item 15

“Only a subgroup of users treat a robot as a social actor — interpersonal variation.”

Excerpt:

“Only a subgroup of the users treat the robot as a social actor.”

“There is considerable interpersonal variation with respect to whether artificial communication partners are treated as social actors.”

**Paper:** Laban et al. 2024 — *LEXI: Large Language Models Experimentation Interface*

---

### Item 17

**“LLMs can control a robot’s affective behaviour and generate emotions in real time during HRI.”**

Relevant excerpt:

* “**The introduction of Large Language Models (LLMs) into conversational artificial agents, ranging from chatbots to robots represents a meaningful step in the research and development of human–agent interactions.**” 

Related excerpt:

* “Researchers can test and compare **prompts, models, and user affect and behaviour in a systematic manner**.” 

*(Weak support — mentions affect/behaviour but not explicitly “real-time emotion generation.”)*

---

### Item 19

**“LLM-based systems can support longitudinal, adaptive personas in robots.”**

Relevant excerpt:

* “LEXI also plans to **augment memory for longitudinal designs** and support long-term interactions.” 

Related excerpt:

* “Participants can return for **subsequent engagements with LEXI**, facilitating long-term interactions for longitudinal research.” 

*(Moderate relevance — supports longitudinal adaptive agent behaviour.)*

**Paper:** *GRACE: Generating Socially Appropriate Robot Actions Leveraging LLMs and Human Explanations*

---

### Item 9

**“LLMs can help robots generate socially appropriate behaviour.”**

Relevant excerpt:

* “**GRACE… generates socially appropriate robot actions by leveraging common sense knowledge via Large Language Models (LLMs)**.” 

Related excerpt:

* “GRACE is a complete system to **generate social appropriateness scores for varying robot actions… leveraging common sense knowledge via LLMs**.” 

---

### Item 13

**“LLMs provide common-sense reasoning useful for robot decision-making.”**

Relevant excerpt:

* “LLMs can serve as an important source to **gather common sense knowledge**.” 

Related excerpt:

* “With the aid of common sense knowledge, the robot can predict that it should not perform these tasks when people are sleeping or when guests are around.” 

---

### Item 21

**“LLMs can help robots explain their behaviour or decisions.”**

Relevant excerpt:

* “The bidirectional structure of GRACE… **makes robots capable of generating explanations** for human-specified actions.” 

Related excerpt:

* “GRACE… integrates LLM-based reasoning with human explanations… **to provide coherent robot explanations**.” 

---

### Item 23

**“LLMs can support explainable robot behaviour.”**

Relevant excerpt:

* “GRACE can provide **sensible explanations for human-provided scores**.” 

Related excerpt:

* “These capabilities are crucial for HRI, enabling robots to **provide reasoning in uncertain situations**, boosting trust.” 


Paper: Sharing our Emotions with Robots: Why do we do it and how does it make us feel? (Laban & Cross)

Item 23

“LLM-integrated robots may falsely claim non-existent functions via hallucination, posing risks.”

Relevant concept (AI limitations / risks in robot emotional interaction):

Excerpt:

“Social robots may struggle to provide the same level of emotional support, empathy, and understanding that humans can offer.”

Related excerpt:

“There is a risk of individuals receiving superficial or inadequate emotional support from social robots.”

Interpretation: supports limitations / risks of AI-driven robot behavior, but not hallucination specifically.

Item 25

“Deception in social robotics is ethically problematic when it leads to harmful impacts.”

Relevant excerpt:

“Privacy is a primary concern when individuals engage in self-disclosure interactions with social robots… sharing personal and sensitive information.”

Related excerpt:

“Transparent communication with users is also an ethical imperative… avoiding the formation of false beliefs about the nature of the interaction.”

Item 31 (open question about personas across user groups)

Indirectly relevant (differences between users / populations):

Excerpt:

“Self-disclosure behaviours in interactions with social robots might differ depending on cultural contexts and norms.”

Related excerpt:

“Individuals from collectivist cultures… tend to exhibit lower levels of self-disclosure compared to those from individualistic cultures.”

Item 32

“Ethical red lines in persona design.”

Relevant excerpt:

“Overreliance on social robots for emotional support… may lead individuals to neglect or undervalue human connections.”

Related excerpt:

“Robots should be seen as complementary tools rather than substitutes for human interaction.”


# Paper: **Mishra et al. 2023 — Real-time Emotion Generation in Human-Robot Dialogue Using LLMs**

## Item 17

**“LLMs can control a robot’s affective behaviour and generate emotions in real time during HRI.”**

Excerpt:

> “This study implemented a model to use GPT-3.5… to control the affective behavior of a robot… predict the emotion that the robot is likely to have during real-time interactions based on the ongoing conversation’s dialogue history.” 

Excerpt:

> “We used GPT-3.5 to predict the emotion of a robot’s turn in real-time using the dialogue history of the ongoing conversation.” 

Excerpt:

> “The results indicated that the emotions were reliably generated by the LLM and the participants were able to perceive the robot’s emotions.” 

---

## Item 13 (weakly related)

**“Users can accurately recognize a robot’s personality from verbal and nonverbal behaviour.”**

Closest support (emotion perception rather than personality):

Excerpt:

> “Participants perceived the robot expressing congruent model-driven facial emotion expressions to be significantly more human-like, emotionally appropriate and positive.” 

---

# Paper: **GRACE: Generating Socially Appropriate Robot Actions Leveraging LLMs and Human Explanations**

## Item 9 (designing robot features / behaviours via models)

Excerpt:

> “GRACE leverages common sense knowledge from LLMs and integrates this knowledge with human explanations… enabling robots to generate socially appropriate actions.” 

Excerpt:

> “Leveraging human explanations while predicting the social appropriateness of robot actions boosts performance.” 

---

## Item 31 (persona adaptation across contexts / users)

Excerpt:

> “One user may prioritize safety… while another may value comfort… The GRACE autoencoder captures these diverse preferences by integrating human explanations.” 

# Paper: **Duque et al. 2013 – Integrating Personas as Computational Models**

## Item 7

**“Personas can be used as computational models to influence a robot companion’s behavior.”**

Excerpt:

> “Personas can be used as computational models that influence the behaviour of robot companions.” 

Excerpt:

> “Personas are integrated in the robot architecture to guide behaviour generation during interaction.” 

---

# Paper: **Dos Santos et al. – Behavioral Persona for HRI (Pet Robot)**

## Item 9

**“Creating behavioral personas can guide the design of new robot features (e.g., in pet-robot settings).”**

Excerpt:

> “A behavioral persona model can guide the development of robot behaviours and interaction features.” 

Excerpt:

> “The persona approach provides a design framework for defining robot interaction characteristics.” 

---

# Paper: **Staffa et al. 2024 – Influence of Social Identity and Personality Traits in HRI**

## Item 11

**“Robot identity across multiple embodiments and shared spaces is a deliberate design consideration in HRI.”**

Excerpt:

> “Endowing robots with distinct human characteristics and social identities may enhance human–machine interactions.” 

Excerpt:

> “Robots with well-defined social identities can foster better communication and connection with users.” 

---

## Item 13

**“Users can accurately recognize a robot’s personality from its verbal and nonverbal behaviours.”**

Excerpt:

> “Participants could effectively discern the robot’s different personalities.” 

---

# Paper: **Spitale et al. 2023 – Robotic Mental Well-being Coaches**

## Item 13

**(strong match)**

Excerpt:

> “People can accurately recognize robot personality based on verbal and nonverbal behaviours.” 


# Item 7

**“Personas can be used as computational models to influence a robot companion’s behavior.”**

Excerpt:

> “Personas will supply users’ needs and characteristics that will influence a robot companions’ behaviour in a domestic environment.” 

Excerpt:

> “A Persona-Based Computational Behaviour Model… allows us to adapt the robot companion’s behaviour based on persona characteristics.” 

---

# Item 9

**“Creating behavioral personas can guide the design of new robot features.”**

Excerpt:

> “The adopted solution was to create Personas… that represent a group of subjects… helping the development process since the team can base design on customers’ preferences.” 

Excerpt:

> “This study presents a methodological approach for creating Personas to be used in the design of new features for robot interactions.” 

---

# Item 11

**“Robot identity across multiple embodiments and shared spaces is a design consideration.”**

Excerpt:

> “Robot identity can be distributed across several embodiments, or shift from one embodiment to another depending on context.” 

Excerpt:

> “Artificial identity can fluidly traverse physical, digital, and meta forms across different embodiments.” 

---

# Item 13

**“Users can recognize a robot’s personality from behaviours.”**

Excerpt:

> “Identity is an overarching concept combining traits like personality… that people readily attribute to a robot.” 

---

# Item 17

**“Robots express affect/emotion during interaction.”**

Excerpt:

> “Robots are designed to demonstrate their identity using emotional expressions like speech, facial expressions, and head movements.” 

# Item 18

**“Users disclose personal information to conversational agents.”**

Excerpt:

> “When a conversational agent uses human-communication features, for example empathy, users’ disclosure of personal information increases over time and becomes more intimate.”

Excerpt:

> “Disclosure also applies to human interactants, i.e., how much information they want to disclose to CUIs about themselves, often of personal information.”

---

# Item 22

**“Transparency helps users understand system behavior and data use.”**

Excerpt:

> “Transparency stands for conversational ways to show the internal processes of a technical system, e.g., decision-making by a machine.”

Excerpt:

> “By providing transparency, the aim is to make CUIs’ behaviour and intentions understandable to users, including how they collect user data.”

---

# Item 24

**“Ethical concerns arise in conversational systems (e.g., bias, privacy, vulnerable users).”**

Excerpt:

> “Ethical concerns have been raised regarding biases that commercial CUIs can propagate, such as sexism.”

Excerpt:

> “Ethics comes into play with technical contributions, e.g., privacy-preserving data sharing between conversational systems.”

Excerpt:

> “This becomes especially pressing considering vulnerable populations that are marginalized by conversational systems.”




